Rules of Engagement: Why and How Companies Participate in OSS

Company engagement in open source (OSS) is now the new norm. From large technology companies to startups, companies are participating in the OSS ecosystem by open-sourcing their technology, sponsoring projects through funding or paid developer time. However, our understanding of the OSS ecosystem is rooted in the 'old world' model where individual contributors sustain OSS projects. In this work, we create a more comprehensive understanding of the hybrid OSS landscape by investigating what motivates companies to contribute and how they contribute to OSS. We conducted interviews with 20 participants who have different roles (e.g., CEO, OSPO Lead, Ecosystem Strategist) at 17 different companies of different sizes from large companies (e.g. Microsoft, RedHat, Google, Spotify) to startups. Data from semi-structured interviews reveal that company motivations can be categorized into four levels (Founders' Vision, Reputation, Business Advantage, and Reciprocity) and companies participate through different mechanisms (e.g., Developers' Time, Mentoring Time, Advocacy & Promotion Time), each of which tie to the different types of motivations. We hope our findings nudge more companies to participate in the OSS ecosystem, helping make it robust, diverse, and sustainable.

==> Acknowledgment.tex <==
\section{Acknowledgments}
Anonymized for blind review. 

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> branding_marketing.tex <==
\textbf{Visibility -D1.5}:

 \MyBox{\textbf{Visibility:} companies participate in OSS because they want to:  
 \begin{itemize}
     \item Increase their visibility
      \item Be credited as the founder of a technology that is now the industry standard (P18)
     \item Positioning their name to the domain they are known for
     Be recognized in their domain of expertise 
     \item Expand or reposition their brand name beyond the domain that the company is known for
    
     
 \end{itemize}} 
 

In open source \inlinequote {the brand recognition is very powerful [P14]} and companies from different sizes participate in open source to increase their visibility (P1, P2, P4-P9, P11, P13-P16)

\boldification{general motivation visibility}
Our interviewees considered Branding/ Marketing as a driver of open source participation (P1, P2, P4-P9, P11, P13-P16). For instance, P14 stressed that in open source \inlinequote {the brand recognition is very powerful}. One interviewee, the OSPO lead at a large tech company, associated open source branding with the branding of the technical ideas behind an app as opposed to the branding of a product as a black box: 

\longquote{P4}{open sourcing these bits and pieces... can help the deal of branding of the technical ideas of an app... and [company name] saw a lot of good press}


\boldification{Visibility, positioning in the domain the company is already known for}
One forms of Branding/Marketing that open source helps with is  visibility (P4, P2, P1, P9, P7, P6, P5, P15, P16) as explained by P2, CEO of a startup whose company is present and active in multiple OSS projects, \inlinequote{and we wanted to be there in our case, because this brings a lot of visibility}.





%their overall visibility, interviewees from large technology companies considered being recognized for standardizing a piece of technology as the ultimate visibility goal (P3, P4, P18):  
%While visibility is a main part of branding
%Branding and marketing has always been at the core of companies' reputation [XX], and open source provides an open transparent platform that helps spread the company's brand. 





\longquote{P4}{ And the best way to do this is to make sure that what you are working on inside of your company, and the thing you depend on actually becomes the industry standard, not just something you maintain... And if you actually came up with this standard, then you also get a lot of exposure.}
 
Our interviewee highlighted as an example the amount of Branding exposure that both Google and Facebook had gained from open sourcing technologies that are now industry standard: 
 
\longquote{P3}{open sourcing React has provided more value for Facebook than leaving it to themselves ever could have. Because A, they get contributions now on that library. B, they get the sort of street credit of the founders of React}


%"where open source is superior is it gives us superior visibility" [P15]

%P2 also emphasize the importance of visibility for a growing startup \inlinequote{the CEO of [large OSS foundation] announced in a keynote [city and name of conference]. We are now Running [OSS community]. And all of these companies and universities are part of this [company name] was there. So that was like great visibility, a really good milestone for us}

%\boldification{showcasing technical achievement and build understanding of what the company already does}

With the visibility that comes with open source, small companies are able to build a brand name  beyond the borders of their country as explained by P6: \inlinequote{We have several views in different countries...started to become more international... a nice way to increase our brand in our company.}

Once a company is relatively visible in the open source space, it can start to build an understanding of what it actually does internally. In fact, interviewees from companies of varying sizes reported leveraging open source to build an understanding of what the company is doing by showcasing their technical achievements (P7, P4, P2, P1) as explained by P4 \inlinequote{so having that open source would be a good contribution to further increase that understanding of what's actually going on inside.} This helps attach the name of the company to their domain of expertise.

\boldification{Vs. repositioning expends the brand name of the company to more than what it is known for}
However, this positioning and understanding is not static as 
interviewees also saw open source as an ecosystem that can expand their brand name beyond what the company has been known for (P11, P2, P1, P4). In particular, open source can help companies transition to a different domain of expertise beyond the one that they have been known for:  
\longquote{P11}{so people tend to think of [company name] as like the people who did [specific product]. And we've really moved beyond that. And so our focus right now is really on building platforms and application developer tool sets that people can use on top of those platforms} 


==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

\boldification{reiterate the importance of this work--similar to part of intro}
Understanding \textit{why} and \textit{how} companies  contribute to OSS provides a complete picture of all OSS players sustaining and maintaining the OSS ecosystem---making space for current and new participating companies to contribute effectively. 

\boldification{interesting examples from results}
Interestingly, our results revealed that though growing and large companies share some motivations, their reasoning may differ. For example, smaller companies reported being motivated by gaining a reputation, since OSS allows them to be in the same space as big-name companies; larger companies reported the same motivation, in this case, because their contributions to OSS signal good citizenship. %Furthermore, Reputation motivation was the most common driver for companies' contributions, with six out of seven of the contribution categories stemming from this motivation.

%\boldification{motivation and contribution categories we identified}
%In trying to understand companies' motivations and contributions to OSS, we empirically identified twelve subcategories of company motivations to contribute to OSS and seven high-level categories of OSS contributions across companies. We analyzed these twelve motivations within the four high-level categories we identified: (1) Founder(s)' vision, (2) Business advantage, (3) Reputation, and (4) Reciprocity, where the Reputation motivation led to six out of seven of the companies' contributions. 

\boldification{what our results provide/contribute summary}
In summary, the main contributions of this paper are (1) a comprehensive model of companies’
motivations to contribute to OSS, (2) a conceptual model showing the multi-faceted ways that companies engage in OSS, linked to their motivations, and the benefiting entities, and (3) lessons learned from companies to foster a healthy OSS-company relationship. 

\boldification{conclude and future}
We hope our results encourage and provide guidance for current and new participants in the OSS ecosystem--specifically companies--to engage in OSS, collaborate in the open, create better software and broaden the economic pie. The lessons we learned from this study will help both companies and OSS projects continue to foster this symbiotic relationship in which they sustain each other effectively.


==> good_quotes.tex <==
And if you're not able to build in the community, then the benefits of open software development and open source are completely zero. There's there's no special benefits to things in the open. It's nice. But it's... there's no there's no reciprocity in some ways, even small, then you're missing the point entirely. [P9]

And it's not just people spending time on code, but also people spending time on people. And so some of our programs that look at more community management and mentorship, that are more about fostering community dynamics, relationships, events, where people can come together and collaborate and meet each other as people I think are seeing that is, can't be discounted, like, I think a lot of the sort of how we contribute back tends to focus too much a bit on the code and engineering aspects.[P20]

% 8:2 ¶ 27 in [P7] Josep-Aiven interview.docx
% obvious one is we consume open source, that's the, the most obvious one, and like 99% of the companies in the world do that.

[start of giving back to dependency]
% 12:9 ¶ 76 in [P15] JoshB RedHat Interview.docx
% Yeah, I mean, usually, right. I mean, for example, the primary reason why we care about products--projects is that they feed directly and intimately into a product line. Yeah, right. So right Kubernetes leads directly to OpenShift container platform, right? The Linux kernel leads directly to Red Hat Enterprise Linux. The and and so we tend to care about those kinds of projects more than we care about sort of ecosystem projects

==> ideas.tex <==
"open source becomes a force multiplier for their cloud business, with open source complements feeding a proprietary core (the core being all the services running on Azure or other clouds)."

"Open source is at the heart of free market software liberalism"  

==> tables/compIndividual.tex <==
\begin{table*}[hbt]
\centering
\footnotesize
\caption{\review{The mapping between the roles presented in this paper and the onion model}}
\label{tab:rolesOnion}
\review{
\begin{tabular}{|l|c|l|}
\hline

\textbf{Roles} & \textbf{Relationship} & \textbf{Onion Model Roles} \\ \hline\hline

\multicolumn{3}{|l|}{\textbf{ \cellcolor[gray]{0.9} Community-Centric}}\\
\cline{1-3}
    


Community Founder/Leader & \textit{encompasses} & Project leader
\\ \hline

OSS Advocate &  \cellcolor[gray]{0.7} & None
\\ \hline

OSS Mentor &  \cellcolor[gray]{0.7} & None
\\ \hline

OSS Strategist & \cellcolor[gray]{0.7} & None
\\ \hline

OSS Treasurer & \cellcolor[gray]{0.7} & None
\\ \hline

OSS Writer & \cellcolor[gray]{0.7} & None
\\ \hline

OSS License Manager & \cellcolor[gray]{0.7} & None
\\ \hline \hline


\multicolumn{3}{|l|}{\textbf{ \cellcolor[gray]{0.9} Project-Centric}}\\
\cline{1-3}

OSS Coder & \textit{encompasses} & Bug fixer, peripheral developer, active developer, core member
\\ \hline

OSS Project Manager & \textit{encompasses} & Project leader 
\\ \hline

OSS System Admin & \textit{encompasses} & None
\\ \hline
%Not included & \textit{encompasses} & Bug reporter
%\\ \hline

\end{tabular}
}
\end{table*}


==> tables/projectsSportsmanship.tex <==
\begin{table*}[bht]
%\footnotesize
%\scriptsize
\caption{OSS Sportsmanship: lessons learned for projects}
\begin{tabular}{p{0.2\textwidth}p{0.1\textwidth}p{0.6\textwidth}}
\toprule
{\textbf{Takeaway}} & {\textbf{Participants}} & {\textbf{Quotes}} \\ \hline

  
%--------------------Projects Takeaway-----------------
\textbf{Avoid toxicity and foster the project's positive environment}
%lower the toxicity of your project have a friendly open project where all contributors are respected and welcomed and interactions are friendly and not toxic 
&
 P5, P7, P10, P15, P18
&

``If it's an abusive community, even companies don't want to get involved. And the other is, is just, you know, companies look at is this a healthy community?'' [P18]
\newline
 ``They [companies] run far away because the moment you see an internet spat or an open source spat, the corporation sees up in like, oh my god, like there is no way we're gonna come out of this good, right because all internet fights... they're like, oh my gosh, step away'' [P10]



%``We are not going to allow our community to create fear, or lack of safety. If you're afraid to ask a question in our community, we're failing. If you're fearful that you're going to look or sound stupid in our community by asking a question, we have not set up our community the right way'' [P5]

\\

%And when you have a set of people that are from different backgrounds, and different incentive structures, and companies and locations, there's a lot of nuance that goes into ensuring that you're fostering a healthy and respectful community. And I think more so I think a lot of what we hope to bring to the table beyond just the funding and the people is support in in these sort of softer dynamics that are vital to the success of any project. So that's more of a lofty goal. But we've been investing in more programs and initiatives that we hope will help to just improve that aspect of things and improve the way that we have we create spaces for people to connect, we have been trying to mentor more people on understanding inclusivity diversity, equity inclusion initiatives, how to have these sorts of conversations, how to have recognition and Ally ship and all these sorts of harder, more difficult personal based dynamics. [P20]

%So projects also need to make it easy for not just company but everyone to contribute, make it a welcoming community, have contribution guidelines, review issues, give proper feedback, of code of conduct, all of those kinds of things. If it's an abusive community, even companies don't want to get involved. And the other is, is just, you know, companies look at is this a healthy community? Is there a proper, you know, cadence to the innovation? Is it maintained by one person, you know, just one person somewhere who randomly will make things happen? [P18]

%You know, something as simple as having a conversation with an organization that helps people learn how to develop. They come from an underserved population, maybe they've never gone to college, or maybe they're doing a career transition, where they've been doing something for 20 or 30 years. And now they want to transition into development. Partnering with those companies to say, who's graduating out of your programs, do they fit our tech stack? We want to talk to them. Right? So creating opportunities for all sorts of developers. Can we ingest a ton of newbies and make them successful? No, not at our scale. Could we take a few? Yeah. We have developers who work in areas of the world that are you know, not quite like the United States. We are making opportunities for developers in countries that are less developed. And we're giving them significant financial freedom. Because we pay them for their contribution, not for what they should be paid in that country. [P5]

%5:11 ¶ 189 in [P5] Jill-SlimAI interview.docx
%And you have to have clearly defined guardrails on what behavior is unacceptable. So when someone is behaving outside of what's acceptable, you also need to take the time to pull them aside and say, This isn't aligned with our community code of conduct or this isn't aligned with our culture and how we communicate? What can I do to help you to get to where you need to be, so that you can contribute? And after you've done that, if they can't opt in, you then very clearly need to say we're not going to allow you to contribute at this time. When you're ready to come back you let us know.

%We have developers who work in areas of the world that are you know, not quite like the United States. We are making opportunities for developers in countries that are less developed. And we're giving them significant financial freedom. Because we pay them for their contribution, not for what they should be paid in that country. [P5]

%Again, it's the idea is not to say like we do this thing, just because people come to us, it's we want to make those ecosystems healthy, welcoming, more attractive for everyone to use and contribute. And if some of these people then come to Aiven, because they heard Aiven is actively doing those things, way better.[P7]


%But for a very successful public open source project, that is one where you have a public community of people, you know, contributing and involved, who work for all kinds of different employers, or no employer or, you know, all over the place. [P15]




%-------------------------------------------------------
\textbf{Have open leadership and governance}
&
 P1, P3, P4, P9, P10, P11, P15, P18 
& 
``Companies can be a little bit reluctant to contribute to open source projects that are owned by companies, because, you know, companies are fickle, we change our strategies, and maybe we stop working on the project and goes away. And or maybe we decide to exert too much control and people get uncomfortable'' [P11]
\newline
``If you do the corporate coalition stuff, you generally need the project to be in a foundation from day one, right?... if you don't have a foundation, then one of the companies needs to own things. And then everyone else needs to trust that one company, which is hard'' [P15]
\\ 

%And this is where I think, you know, foundations like the Apache Foundation, the Linux Foundation, become really good neutral homes, for companies to come together to collaborate. If five cloud companies have the same challenge, it makes sense to work together to solve that problem, and not solve it through partnerships and agreements, because that's a very heavy legal lift. But to come together in a foundation and to say, let's create a charter, that's, you know, maybe one company has started solving that problem, and then release that code to that foundation, when everybody else starts working on that, and can continue to improve that.[P18]

%4:31 ¶ 87 in [P1] Georg-Bitergia interiew.docx
%So Bitergia started the grimorelab project and built a community around the metrics. So Grimoire Lab is the metrics tool that we have. And we had Grimore con, which is event series of bringing people together who wanted to talk about metrics and using Grimoire Lab to get metrics. And and then Bitergia was looking okay, how do we, how do we grow that community more? What What can we do? And so we approached the Linux Foundation to say, hey, Linux Foundation, you're hiring us for getting the metrics, you're using the tools. You also host projects, can you host Grimore lab, as a project as a Linux Foundation project? And the Linux Foundation said, yeah, we can do that. And we also have these researchers at the University of Nebraska, who are doing metrics work, who want to understand Project Health, you have the tools Bitergia let's bring this together and create one community. And so Bitergia Research Group Linux Foundation, we all sat together decided to name this one group chaos. And so chaos is the next step from the Bitergia perspective of the community that we have built. But now, chaos has a bigger scope, than just metrics around the Grimoire Lab tool because now there's also research interest they have the research project. And it's bigger. It's bigger pie with what we are doing as part of that.

%1:17 ¶ 105 in [P3] Omer-VM interiew.docx
%Exactly, exactly. And then when you are collaborating, right, so Knative is about to be donated to the CNCS. That took a lot of work to get to happen years of lobbying and politicking and striking and it's so much stuff, because the vendors that are involved in that project already have representation in these foundations. So in their mind, they would like to put these things where they already have influence, and in a place that they can trust that other vendors won't screw them over. And the CNCF and Linux Foundations have done a pretty good job of being like, Okay, we are a neutral home for these things.

%2:40 ¶ 109 in [P4] Per-Spotify interview.docx
%So we have no involvement other than like, some, I think some people do get involved in like, [inaudible], it's very individual decision based on their needs. So Spotify do not have a strategy of influencing the projects that depend on. It happens on a per dependency basis, if, if an engineer sees like a need to raise a discussion with our team, they will do so. But no, we don't we don't have we don't have a plan to leverage ourselves as a company to to influence our dependencies. A

% it benefits you to have advisors who are also experts in that ecosystem. So we have folks like Kitt Marker and Brendan O'Leary and Kelsey Hightower and Alan Chisa, we have people in the extended ecosystem, who are advisors who spend regular time with us to help us guide the strategy and execution of the business in a way that is appropriate for the ecosystem. Right? When you behave that way, both internally and externally, you can produce more faster, because it's not just us internally doing it. The amplification is way bigger. Mm hmm. Right. And so and so if we, it's not just us talking about us, its advisors, its investors, its users, right. So it amplifies out bigger and faster.[P5]

%10:34 ¶ 160 in [P9] Phillipe NexBe Interview.docx
%And now, in selecting code, a library that we use, that will be critical dependencies for us, that will be typically be a serious criteria. If we think it's important for us to participate in the governance, and we're not allowed to, we would probably just pass and move on to something else and not use the code at all. There's example like that I wouldn't give specific name. But there's a project with which we were involved fairly significantly. And it was very clear that nobody was welcome to provide input on on the governance and directions of the project. So we passed, we disengage, and we disengage completely, basically... So there's there's one possible challenge, but it's more of a problem. That's the only challenge maybe free riding. Which is if you do free riding. Which means when you have contributors, well, users that that eventually abuse and free ride without ever contributing back.[P9]

%And that becomes a very important part of how open source modern open source grows. It's not the weekend warrior. I mean, in some cases, it is but for a lot of cases, it's not a weekend warrior, that's going to create Kubernetes it's Google, who going to pay engineers full time all day every day and feed them to make a technology and then strategically give that to a foundation to grow in public, so that more people use a technology and oh, by the way, they have a cloud providing service that you pay for that, you know, has some sort of consistency with with that technology. [P10]

% And the question is, who owns the intellectual property of the joint venture? So if I have a joint venture, some some of my people, some of you people are, are coming together to create something? Well, somebody has to own the output, it's either one entity owns it, the other entity owns it, it's owned in a joint way. Or it's given to some sort of neutral sort of neutralized status. Those are sort of your basic four outcomes. Well, you want to decide that before you put people in. But last thing you want to do is put people into the fight, and then have a company say we own it. [P10]

%But for us, one of the things that we look at as the primary benefit is really being able to build an ecosystem around the project and build more of a community around the project. Because people can be companies can be a little bit reluctant to contribute to open source projects that are owned by companies, because, you know, companies are fickle, we change our strategies, and maybe we stop working on the project and goes away. And or maybe we decide to exert too much control and people get uncomfortable.[P11]

%I mean, a lot of times that they use, so for example, if you do the corporate coalition stuff, you generally need the project to be in a foundation from day one, right? Because, because, like for a single company, project, that single company can keep paying for the project's resources, you know, and hosting things, etc. And gradually, you know, gradually alienate those items. Right, so gradually, you know, give them up to some sort of public resource or, or you know, come up with a way to have them sponsored or put it in a foundation or whatever, right? There's a flexible timeline around that with one of these corporate coalition's you pretty much need to do it immediately. Because if the CO if you don't have a foundation, then one of the companies needs to own things. And then everyone else needs to trust that one company, which is hard.[P15]
  
\bottomrule
\end{tabular}
\label{table:projectSportsmanshipTable}
\end{table*}


%[other quotes]
%o I think like having, using the policies, like having the right policies and guidelines in their project description, like, you know, like the contributing Markdown file, like how to contribute to the project, also all the policies in place in terms of so they like the sign, like, like the license, for instance, like having a document of which license it is because companies won't be contributing to your project, if there is no license sewing, even though you have it on a GitHub or an anti lab doesn't look doesn't mean that it's open source. So yeah, in overall, it's more like having all these documentation documented in the right place. So I make it easier for companies or individuals as well, to be able to take a look at that. Because they might be like also having like automation, automating tools to review all this. So used to be making sure that you're using the right syntax, and you're putting it in the right place. Because if not, it might be like your open source project. Maybe that just because it's not in the right place. And they're not going probably in my project review. And it's they have their own automation tools. [P19]

%[P18] That's a really, really good questions. One of the reasons why sometimes companies don't contribute is because the project makes it so difficult to contribute either. The, there's no proper guide to contribution, there's no coding guide, there's no readme. A there's no proper license. And so the company has to work extremely hard to find out, you know, how do I come to contribute to this. And that could be bias in the project, also about accepting contributions from certain companies or, or to protect, you know, their own direction, or they may see companies as pushing the company agenda and not thinking about the project in general. So projects also need to make it easy for not just company but everyone to contribute, make it a welcoming community, have contribution guidelines, review issues, give proper feedback, of code of conduct, all of those kinds of things. If it's an abusive community, even companies don't want to get involved. And the other is, is just, you know, companies look at is this a healthy community? Is there a proper, you know, cadence to the innovation? Is it maintained by one person, you know, just one person somewhere who randomly will make things happen? And, I mean, companies can do a lot more here as well, if it's really a valuable project, and it's struggling for maintenance. Companies should help, you know, with the maintenance and not just the feature functions, but the heavy lifting of code reviews and maintaining the project and doing the security and the plumbing. And I would say those are some of the things that projects could do. [P18]

==> tables/visibilityTable.tex <==
\begin{table}[htb]
%\footnotesize
%\scriptsize
\caption{Reputation: Visibility}
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{p{0.2\textwidth}p{0.1\textwidth}p{0.2\textwidth}}
\toprule
{\textbf{Visibility}} & {\textbf{Participants}} & {\textbf{Example}} \\ \hline
  
%____________________Visibility_________________________

Cement their name to their domain of expertise 


&


P4, P7

 
&
  


``Open sourcing these bits and pieces of whenever you can make it like tangible and like very transparent about what was actually going on inside of the company. So that can that can help the deal of branding... And [company] saw a lot of good press'' [P4]


\\
%And, and where open source is superior is it gives us superior visibility into our own supply chain. Right as in, we don't have to-- with proprietary software, you know, if we have a proprietary component, like we were proprietary, authentication component, and we're like, hey, is this being maintained in the light of new security exploits? Right? In that case, you have to trust the vendor to know whether or not that's being maintained. [P15]

%So two reasons. One is personal. And one is business, the personal reason is that we whoever is engaged in in these communities may have a personal interest wants to be wants to learn something new wants to be recognized as, as a leader in that space. So it's a little bit like personal branding. So one, for example, I'm involved in the IEEE sa open community advisory group. And part of that is to build up my credentials as an open source strategist and being an expert on open source communities. For Bitergia, as a company to encourage this and do this, is because being active in open source communities, gives us access to decision makers, at companies that could potentially be customers. And so we use this also as a way for finding prospects and generating business for the company. And most of the business that we do have came through contacts that we fostered in being active in these communities.[P1]

%%2:101 ¶ 23 in [P4] Per-Spotify interview.docx
%So like open sourcing these bits and pieces of whenever you can make it like tangible and like very transparent about what was actually going on inside of the company. So that can that can help the deal of branding of the technical ideas of an app like Spotify, I think. And Spotify saw a lot of good press with like this, Spotify wrapped the day over the Christmas period where everyone got like the year overview of music. And that kind of thing took like a ton of machine learning a ton of data and a lot of engineering tricks, to do this little little feature. And so this is like this is one of the ways they want to be more transparent about like, how do we actually use these, like very sophisticated systems of understanding music and user behavior and, and music history and so on. So we can kind of create this little feature called wrapped, which is just one month a year. 

%8:125 ¶ 135 in [P7] Josep-Aiven interview.docx
%write articles on presence while trying to showcase what we do share the Word of either what we do at Aiven, what we do in the open source space, how we shape things. 

%8:72 ¶ 71 in [P7] Josep-Aiven interview.docx
%Because they were asking if we have some experts on X, Y, Z? And then it's like, yes, we have some. So of course, you can claim to be an expert, if you contribute regularly to a project, yes, kind of probably.

%-----------Expand brand beyond domain-------------  

Expand their brand beyond the domain that the company is known for 

&

P4, P11

&

``So people tend to think of [company name] as like the people who did [specific product]. And we've really moved beyond that'' [P11]

\\ 

% ``open sourcing these bits and pieces of whenever you can make it like tangible and like very transparent about \\ what was actually going on inside of the company. So that can that can help the deal of branding [P4]''

%2:56 ¶ 19 in [P4] Per-Spotify interview.docx
%just like branding, like that a company, what they do, again, what they do inside is not very visible on the tech side, like a like an app like Spotify, it's actually quite hard to understand, like, how it actually works, technically. And why should that even be interesting? For many doing point of view, if you're like a top notch engineer at Google, or Facebook or Apple, why should you work at Spotify? It's just like an app that plays music.

%9:9 ¶ 16 in [P11] Dawn-VM Interview.docx
%so people tend to think of VMware as like the people who did virtual machines. And we've really moved beyond that. And so we-- well our focus right now is really on building platforms and application developer tool sets that people can use on top of those platforms to build their applications. So we do that across all the clouds

%---------Be credited as founder of technology-------------

Be credited as the founder of an industry standard technology
 
&

P3, P4, P13-P15, P18

&

 ``Business that decides to release a project because they want to create a standard in the world around that particular software... %, like, you know, Google did with Kubernetes, it became the de facto \\ way to do container orchestration... 
 And the company that created it and released it has an advantage, because they are seen as thought leaders'' [P18]

\newline

``Google got a lot of exposure from like, creating Kubernetes, which is like the industry standard for like management services'' [P4] 
\\

%It could also be a business that decides to release a project because they want to create a standard in the world around that particular software, like, you know, Google did with Kubernetes, it became the de facto way to do container orchestration, as and so many other projects have become kind of the de facto standard for doing something. And the company that created it and released it has an advantage, because they are seen as thought leaders, people want to join them from a recruitment perspective.[P18]

%``the best way to do this is to make sure that what you are working on inside of your company... \\becomes an industry standard, then you gain all the benefits from being part of the standards. And if you\\ actually came up with this standard, then you \\ also get a lot of exposure. [P4]%Like Google got \\a lot of exposure from like, creating Kubernetes, which is like\\ the industry standard for like management services'' 

  %``If you actually came up with this\\ standard, then you also get a lot of\\ exposure... And is again it kind of\\ is like our desire to be able to be\\ a standardized piece of \\technology''[P4]
 

%  ``if you actually came up with this standard, then you also get a lot of exposure... And is again it kind of is like our desire to be able to be a standardized piece of technology''[P4]

%2:51 ¶ 37 in [P4] Per-Spotify interview.docx
%And if you actually came up with this standard, then you also get a lot of exposure. Like Google got a lot of exposure from like, creating Kubernetes, which is like the industry standard for like management services. Now again, and Spotify wants to kind of create the same kind of narrative for like internal

%2:90 ¶ 97 in [P4] Per-Spotify interview.docx
%h, yeah. And is again it kind of is like our desire to be able to be a standardized piece of technology instead of just an esoteric Spotify technology

%17:11 ¶ 88 in [P14] Harish RedHat Interview.docx
%And then the Linux kernel community, eventually settled on the model that we had also adopted. We already had adopted. And so guess what happens? The SUSE guys had to scramble, because now they have a kernel that is only using that type of threading which the upstream is not accepting. They say, yeah, it doesn't make sense. And so they had to scramble and I know of customers who were abandoned by SUSE because they were already going down that path, which was not the right path to go and SUSE couldn't quickly, you know, re engineer the stuff so that they can so they have to sunset that portion of the tech so that they can go into the newer threading model in the kernel. So. So that's the kind of benefit that we get as an example. So benefit, right?

%18:37 ¶ 298 – 302 in [P13] Tobie OSS consultant Interview.docx
%Yeah, it's a lot of money. Yeah. Um, and so that was just essentially by commoditizing. The layer under what it is that they were serving
%[R] So this is Facebook being able to save that amount by by standardizing
%[P13] by essentially open sourcing, sort of like the structure and diagrams of how they were making. 

%18:38 ¶ 296 in [P13] Tobie OSS consultant Interview.docx
%But let's say that they realize they could make a lot more money selling hardware than, than selling their software. Right. They could make the whole zoom thing, completely open source, for example. And make it work extremely well with their hardware. So that Sure, they would lose money and have like, fewer people actually paying for it, but they would become the de facto solution for all hardware, built on for, you know, whether like, regardless of who was using that system or not. 

%1:13 ¶ 187 in [P3] Omer-VM interiew.docx
 %the sort of street cred of the founders of React,

%1:19 ¶ 187 in [P3] Omer-VM interiew.docx
%get an entire class of engineers, who are now familiar with the tech stack that Facebook uses, right? Or at the very least, like one of the main web frameworks that they're using, that they have sort of home grown, right. And they also get viewed as, like a cooler place to work. 

%2:58 ¶ 37 in [P4] Per-Spotify interview.docx
%They, they want to leverage open source as much as possible. And the best way to do this is to make sure that what you are working on inside of your company, and the thing you depend on actually becomes the industry standard, not just something you maintain. Because if it becomes an industry standard, then you gain all the benefits from being part of the standards. And if you actually came up with this standard, then you also get a lot of exposure. Like Google got a lot of exposure from like, creating Kubernetes, which is like the industry standard for like management services. Now again, and Spotify wants to kind of create the same kind of narrative for like internal 

%12:16 ¶ 130 in [P15] JoshB RedHat Interview.docx
%But you know, have partners and customers that are using it. Yeah. And you don't want to piss them off. By terminating the tool? Well, if it's open source, you can just kind of gradually pull all your engineers off of it, and let them have it. Um, you know, so this is what's called the abandonware strategy. Now, that that's generally used as a derogatory term, but sometimes abandonware is good, right? Because it's something we can do with open source that you could never do with proprietary software, where you say, Hey, I know you guys are still using this. I know you still like it, but it doesn't make any sense for us as a business anymore. So here, it's yours. Now you can have it.

  
\bottomrule
\end{tabular}}
\label{table:visibilityTable}
\end{table}

%-------------General Visibility Quotes-----------------

%``Where open source is superior is it gives us superior visibility'' [P15] 

%``We decided to do is write a blog post... Well, a bunch of people started commenting on that. And it raised awareness of [company name] because we wrote it, but we didn't mention [company name], really, in that entire article... so it's actually a great marketing tool to talk about technology to use, even if it doesn't promote your, your own product'' [P8] 

%  ``Having companies involved can also help you with... marketing, right?... that helps give visibility to some of these these projects as well'' [P11]

%4:11 ¶ 27 in [P1] Georg-Bitergia interiew.docx
%hey hire us for the expertise. Because we have worked with a lot of open source projects, and foundations and companies that we are really good at knowing what the data is, what is available, what kind of questions we can answer.

%3:18 ¶ 73 in [P2] Daniel-Bitergia interview.docx
%contributing to open source is about demonstrating that you have the expertise and the knowledge contributing, and then you can serve specific pieces of knowledge.

%3:21 ¶ 73 in [P2] Daniel-Bitergia interview.docx
 %So then we can mess with your inner source effectiveness, let's say. But then at the same time, we are serving with the community. So we are defining inner source. So it's not that we know about inner source is that we are defining inner source and for this you can see that we have this pattern here about the maturity model, this pattern there about this or that and then we have these presentations at the inner source commons.


%[visibility/positioning in community]

  %\makecell{Some really \\ longer text}
  %the CEO of [large OSS foundation] announced in a keynote [city and name of conference]. We are now Running [OSS community]. And all of these companies and universities are part of this [company name] was there. So that was like great visibility, a really good milestone for us[P2]
  
  %You know, the other benefit that sometimes people see is you know, having having companies involved can also help you with I don't know, like, I guess marketing, right? So so we have, you know, we have relatively popular blogs and social media channels, and we can promote things about some of the open source projects that we're working on. And that that helps give visibility to some of these these projects as well. So I guess visibility is what I was talking about sovereignly I guess I guess it's marketing.[P11]
  
  %7:22 ¶ 47 in [P8] Johnathan-Goliath interview.docx
%And so we decided to do is write a blog post saying, here's all the things here's how you might want to use JSON, the JSON library in Zephyr, and oh, here's some gotchas we found. Well, a bunch of people started commenting on that. And it raised awareness of Goliath because we wrote it, but we didn't mention Goliath, really, in that entire article. And the maintainers of the Zephyr project, want to see how we can start to contribute back. So that material, so it's actually a great marketing tool to talk about technology to use, even if it doesn't promote your, your own product. And so we're seeing that by by proxy of doing it. 

  
  %So we have a branding, we have collateral point of bringing more people hire more people keep more people here. Get more engaged with more companies that might be the future partners. For example, last year, we had several conversation with Red Hat, who is a huge company about open source. And yes, he has a lot of money. And because of this conference discussion, right now, we had strategic discussion to do more business together. And everybody was everything was based in the first open source commit and open source community discussion. So yes, there is no money directly on those open source products, but it's your work to keep it that's why Zup is zookeeping it so with branding, it's kind of like that.[P6]
  
  %Definitely, I suppose in the marketing and branding level, that the marketing and branding folks always have, like, how is this contributing to our-- I don't work necessarily at that level. But I think that the level we do work at is we want to show up as in some of the ways I was talking about like humble, sincere, dedicated, more than a lot of time brand is about being like when I hear marketing and brand I hear, "we're the best at this look at us" you know, and I don't think that's what we're going for at all. I mean, occasionally, occasionally, somebody might be proud of something, but we're really looking to be part of something. Our brand is being part of something and not the best at something, [P17]
  
  %So we need to use other marketing efforts to be known and to be to be seen out there being being an open source company, I think, helps build like trustable branding.[P2]
  
 %12:3 ¶ 26 in [P15] JoshB RedHat Interview.docx
%The the second way that we're involved with with open source is community. As in open source projects, collect people around them, which are known as open source communities. And open source communities are a good way for us to reach people. It's a major portion of our marketing picture, when I'm talking about marketing with a big M. The and and they supply a lot of sort of key inputs to marketing, you know, both not just, you know, people to basically advertise to, but also as a way of learning what is it that people want, so that we can actually build those products? Right. Um, so marketing in terms of market research, and in terms of getting direct feedback? You know, like, if we're thinking about something new in Linux, we can put it in fedora and see how it does in fedora. Um, you know, before we have to offer five years of support for it.

  
  %7:13 ¶ 31 in [P8] Johnathan-Goliath interview.docx
%It's more about being able to have our voice heard, emphasis on priorities for our company, but also to drive the general shift. Like, because I participate in the marketing side, I'm able to make the marketing efforts better, like, "oh, maybe we should go talk to these people. Or maybe we should have this change the conference upcoming." And so I wouldn't have that opportunity if I wasn't a project member.

  
  %6:47 ¶ 159 in [P6] Otavio-Zup interview.docx
%We have several views in different countries for up to the company. So right now we have I don't know the number but 20,000 views around the globe. We have several countries don't have the right number right now.

%6:73 ¶ 159 in [P6] Otavio-Zup interview.docx
%And how can we engage money from the open source products basically first with brand thanks to the four open source products.

 %3:17 ¶ 73 in [P2] Daniel-Bitergia interview.docx
%we need to use other marketing efforts to be known and to be to be seen out there being being an open source company, I think, helps build like trustable branding.

 %5:74 ¶ 213 in [P5] Jill-SlimAI interview.docx
%Could branding make it easier? Sure. I mean, it might make it more easily recognizable. Yeah. Are there open source projects on market today that don't look anything like their corporate sponsors? Yes. Are there some that do? Yes.

  
 %3:19 ¶ 73 in [P2] Daniel-Bitergia interview.docx
%Yeah, so So the, the open source communities we are part of, we can see them as a way to position branding, to partially use their marketing efforts into reaching out other people that they need, for instance, metrics, or open source metrics, or they need to measure PlayerHealth. And then they go to, to grimoire lab-- to CHAOSS, and they say, well, there is there is a university running or so we I can I can hire them or I can hire, Bitergia for more, you know, professional services or industrial services. Good. So this is like a good place where you can go and fish for potential customers. It

%17:25 ¶ 16 in [P14] Harish RedHat Interview.docx
%So to answer the question is, what is in it for Red Hat? The brand recognition, oh, the guys in Red Hat, they advised us to try to do this. Yeah, they did help us out, we did not pay them all, we paid them something. Oh, do we didn't buy the subscription from them. All, we bought some subscription for them, because we were glad that they helped us, you know, so the leaves hopefully leaves a positive, a positive impression with the organization. Because they have a lot of them, they immediately start comparing us against, for example, I'm picking the name because a very common name, Oracle, or Microsoft, or they just want to, they just come here to make money. They want my money, they want to do this, No, they won't give me anything else. But when they come here, they also want my money, but they also give me other things. And it's okay, even if I don't, even if I don't subscribe to their services, even if I don't buy their service, they're still friendly to me. Whereas the other guys, Oh, you didn't buy from me, I'm walking away. So it's a very different, it's a very human thing. I mean, it's not a it's not a win, win lose environment, it's a win win environment. So you know, in order for the other side to say, oh, I need to win this customer, that means the customers lose the money to me.

%19:19 ¶ 65 in [P16] Stephen Transcribed Interview.docx
%doing good, looks good. And looking good, has, you know, has a potential positive effect on your bottom line? Right. So I think, I think that's definitely one component of it for for enterprises. Participating in open source, like, it looks good to be doing good. 

%19:20 ¶ 65 in [P16] Stephen Transcribed Interview.docx
%making sure that we're, we try to be equitable with the way that we've maintained some of these things within, within smaller parts of various foundations. But also realizing that there's a component of it, that you have to show people why they should care about you.
